CodeFort: Robust Training for Code Generation Models

Code generation models are not robust to small perturbations, which often lead to incorrect generations and significantly degrade the performance of these models. Although improving the robustness of code generation models is crucial to enhancing user experience in real-world applications, existing research efforts do not address this issue. To fill this gap, we propose CodeFort, a framework to improve the robustness of code generation models, generalizing a large variety of code perturbations to enrich the training data and enabling various robust training strategies, mixing data augmentation, batch augmentation, adversarial logits pairing, and contrastive learning, all carefully designed to support high-throughput training. Extensive evaluations show that we increase the average robust pass rates of baseline CodeGen models from 14.79 to 21.74. We notably decrease the robustness drop rate from 95.02% to 54.95% against code-syntax perturbations.

==> sections/context_sensitive.tex <==
Model: $\model{}$, original input prompt: $\bfx$, perturbed input prompt $\perturbed{\bfx} \in \perturbation(\bfx)$, model output on original input prompt: $\model{}(\bfx) = \bfy$, model output on perturbed input prompt: $\model{}(\perturbed{\bfx}) = \perturbed{\bfy}$.

\section{Context-Sensitive Alignment}

The context-sensitive perturbation requires the code generation model $\model{}$ to generate \emph{different} token sequences, while satisfying certain \emph{constraint} for an original prompt and its perturbed version.
In this paper, we focus on a special type of context-sensitive perturbation called rename perturbation that renames a variable or a function name in a program. 
Let $\perturbation_\mathrm{rename}(\bfx) = \{\substitution_1(\bfx), \substitution_2(\bfx),\ldots,\}$ be the set of all possible perturbed prompts from $\bfx$ by the rename perturbation $\perturbation_\mathrm{rename}$, where $\substitution_i$ is a function substituting old names with new names. 
Each perturbed prompt $\perturbed{\bfx} \in \perturbation_\mathrm{rename}(\bfx)$ corresponds to a name substitution $\substitution$, i.e., $\substitution(\bfx)=\perturbed{\bfx}$.
\begin{example}
Consider the following code snippet $\bfc$, ``def identity(x): return x'', if we apply the rename perturbation $\perturbation_\mathrm{rename}$ to this snippet, one possible perturbed snippet $\perturbed{\bfc}$ would be: ``def identity(a): return a'', where the variable name ``x'' is substituted by ``a''.
The perturbed snippet $\perturbed{\bfc}$ corresponds to a substitution $\substitution_{x\mapsto a}$, i.e., $\substitution_{x\mapsto a}(\bfc)=\perturbed{\bfc}$.
\end{example}

Given the original prompt $\bfx$, the perturbed prompt $\perturbed{\bfx}$, and the corresponding substitution $\substitution$, the constraint of rename perturbation $\cons_{\perturbation_\mathrm{rename}}$ requires the generation of the perturbed prompt $\perturbed{\bfy}$ to be the same as the original generation $\bfy$ after applying the substitution $\substitution$.
Formally, $\cons_{\perturbation_\mathrm{rename}}(\bfy, \perturbed{\bfy})$ is defined as $\substitution(\bfy)=\perturbed{\bfy}$.

\begin{example}
Let $\bfx$ = ``def identity(x): '', $\perturbed{\bfx}$ = ``def identity(a): '', and the expected outputs for model for two prompts be $\model{}(\bfx)=\bfy$ = ``return x'', $\model{}(\perturbed{\bfx})=\perturbed{\bfy}$ = ``return a''.
These two expected outputs satisfy the constraint $\cons_{\perturbation_\mathrm{rename}}$ because $\substitution_{x \mapsto a}(\bfy)=\perturbed{\bfy}$.
\end{example}

\subsection{Context-Sensitive Alignment}
In context-free alignment, we design our loss functions to encourage the model compute the same hidden states for the original prompt and the perturbed prompt.
However, the context-free alignment does not work for context-sensitive perturbation because from the same hidden states, the model will generate same output sequences which contradict the requirement of the context-sensitive perturbation. 

\yh{Why not use [MASK] tokens to ``neutralize'' the influence of the substituted variable/function name? It's a good idea, I plan to try out it later.}

Given the following original prompt $\bfx = x_1, x_2, \ldots, x_{k-1}, x_k$ and its perturbed version $\perturbed{\bfx} = \perturbed{x_1}, x_2, \ldots, x_{k-1}, \perturbed{x_k}$\footnote{To simplify illustration, we only consider the case where two tokens $x_1$ and $x_k$ have been substituted.}, we denote the model hidden states after seeing $\subseq{\bfx}{1}{i}$ and $\subseq{\perturbed{\bfx}}{1}{i}$ as $h_i$ and $\perturbed{h}_i$.
The hidden state $h$ contains two information 1) $h_{name}$, the information related to the identifier that will be substituted, e.g., what is the name of this identifier, and 2) $h_{null}$, other information that is orthogonal to the identifier, e.g., the overall program control flow.


\begin{assumption}
\label{eq: addable}
We assume that the sum of this two information vector $h_{name}$ and $h_{null}$ gives back the hidden state $h$.
Note that we do not assume that $h_{name}$ and $h_{null}$ are orthogonal because $h_{name}$ might contribute to $h_{null}$, e.g., a variable name ``i'' has a large influence to the program control flow. 
We further decompose $h_{name}$ as $h_{name\_mere}$ and $h_{name\_null}$.
$h_{name\_name}$ contains mere information about the name of the variable and it is orthogonal to both $h_{null}$ and $h_{name\_null}$.
Formally,
\begin{align}
    h = h_{name\_mere} + h_{name\_null} + h_{null},\quad h_{name\_mere} \perp h_{name\_null} \wedge h_{name\_mere} \perp h_{null}
\end{align}
\end{assumption}
In context-sensitive alignment, we want to keep the difference between $h_{name\_mere}$ and $\perturbed{h_{name\_mere}}$ and to align $h_{null} + h_{name\_null}$ and $\perturbed{h_{null}} + \perturbed{h_{name\_null}}$.
\yh{A stricter version is to only align $h_{null}$ and $\perturbed{h_{null}}$, but it is hard to filter out the name contribution $h_{name\_null}$. Note that the original name contribution $h_{name\_null}$ might be better than $\perturbed{h_{name\_null}}$, e.g., in VarRenamerRN, a meaningful variable name will be replaced by a random valid variable name.}

\subsubsection{Disentangle $h_{name\_mere}$ from $h$}
The key challenge of context-sensitive alignment is to disentangle $h_{name\_mere}$ from $h$. 
\begin{assumption}
\label{eq: sameness_across}
Between two occurrence of the substituted name, say, $x_1$ and $x_k$ ($\perturbed{x_1}$ and $\perturbed{x_k}$, respectively), each $h_{i,name\_mere}$ in $h_i$ should be the same for $1\le i <k$.
\end{assumption}

\begin{corollary}[Adjacent disentanglement from Assumption~\ref{eq: sameness_across}]
\label{eq: adjacent}
For all $1 < i < k$, let $g_i = h_i - h_{i-1}$, then $g_i \perp h_{i,name\_mere} \wedge g_i \perp h_{i-1,name\_mere}$.
\end{corollary}

Corollary~\ref{eq: adjacent} holds when $\forall 1< i < k.\ h_{i,name\_mere}=h_{i-1,name\_mere}$, which is equivalent to Assumption~\ref{eq: sameness_across}.

\begin{corollary}[Average disentanglement from Assumption~\ref{eq: sameness_across}]
\label{eq: average}
Let $g_i = \frac{1}{k-1} \sum_{j=1}^{k-1} h_j - h_i$, then $\forall 1\le i < k.\ g_i \perp h_{i,name\_mere}$.
\end{corollary}

Corollary~\ref{eq: average} holds when $\forall 1\le i<k.\ h_{i,name\_mere}=\frac{1}{k-1} \sum_{j=1}^{k-1} h_{j,name\_mere}$, which is also equivalent to Assumption~\ref{eq: sameness_across}.

Using Corollary~\ref{eq: adjacent} or Corollary~\ref{eq: average}, we can identify a vector $g_i$ that is orthogonal to $h_{i,name\_mere}$. We can use $g_i$ to disentangle $h_{i,name\_mere}$ from $h$ by projecting $h_i$ onto $g_i$.
\begin{theorem}
\label{theorem: disentaglement}
\begin{align}
    h_{i,name\_mere} = h_i - \frac{\langle g_i, h_i \rangle}{\|g_i\|\|h_i\|} g_i, \quad h_{i,null} + h_{i,name\_null} = \frac{\langle g_i, h_i \rangle}{\|g_i\|\|h_i\|} g_i \label{eq: disentanglement}
\end{align}
\end{theorem}
Using Theorem~\ref{theorem: disentaglement}, we can get $h_{i,null} + h_{i,name\_null}$ for the original prompt and get $\perturbed{h}_{i,null} + \perturbed{h}_{i,name\_null}$ for the perturbed prompt.
We then use contrastive loss to align $h_{i,null} + h_{i,name\_null}$ and $\perturbed{h}_{i,null} + \perturbed{h}_{i,name\_null}$.
\yh{Do we need to make sure the assumption 1.2 holds? We can compute $h_{i,name\_mere}$ from Theorem~\ref{theorem: disentaglement} as well, we can design loss to ensure $h_{i,name\_mere}$ are all the same for all $1 \le i <k$.}


==> tables/equations.tex <==
% \begin{table*}
%     \centering
%     \begin{tabular}{l}
%          \toprule
%          Equations\\
%          \midrule
% \begin{align}
% \lossdataaug = \sum_{j=1}^b a_j\lossclm(\trpoint{\pt{\bfx}}{j}) + (1-a_j)\lossclm(\trpoint{\bfx}{j}), \label{eq: lossdataaug}
% \end{align}
% \\
%           \\
%          \bottomrule
%     \end{tabular}
%     \caption{Definitions of the robust training losses.}
%     \label{tab:my_label}
% \end{table*}


\begin{figure}
\small
    \begin{align}
        \lossdataaug = \sum_{j=1}^b a_j\lossclm(\trpoint{\pt{\bfx}}{j}) + (1-a_j)\lossclm(\trpoint{\bfx}{j}), \label{eq: lossdataaug} \\
        \lossmdataaug = \sum_{j=1}^b a_j\lossclm(\trpoint{\pt{\bfx}}{j}, \trpoint{\pt{\mask}}{j}) + (1-a_j)\lossclm(\trpoint{\bfx}{j}),  \nonumber\\
        \lossmbatchaug = \sum_{j=1}^b a_j\lossclm(\trpoint{\pt{\bfx}}{j}, \trpoint{\pt{\mask}}{j}) + \lossclm(\trpoint{\bfx}{j}) 
    \end{align}
    \caption{Definitions of robust training losses.}
    \label{tab:loss_defs}
\end{figure}

==> tables/motivation_small.tex <==
% \usepackage{tabularray}
\begin{table}
\setlength{\tabcolsep}{3pt}
% \renewcommand{\arraystretch}{1.}
\centering
\caption{We evaluate the robustness of SOTA public code models on ReCode~\citep{recode} benchmark. Under four types of semantic-preserving program transformations on the same MBPP evaluation set, we see significant drops of pass@1 rate over unperturbed ones. The results indicate unsatisfied robustness performance of SOTA models.}
% \myshang{This table and its caption are not very clear to me. what's the baseline that the drop in this table is comparing against? (todo: codegen16B)}\linbo{Maybe adding one column: clean accuracy?}
\vspace{-0.5em}
\resizebox{0.9\linewidth}{!}{
\begin{tabular}{lllll}
\toprule
Models & Docstring & Function & Syntax & Format\\
\midrule
StarCoder-15B & 71.89\%$\downarrow$ & 62.93\%$\downarrow$ & 92.91\%$\downarrow$ & 60.21\%$\downarrow$ \\
WizardCoder-15B & 61.66\%$\downarrow$ & 45.47\%$\downarrow$ & 83.86\%$\downarrow$ & 53.95\%$\downarrow$ \\
% CodeLlama-7B & 78.70\%$\downarrow$ & 69.37\%$\downarrow$ & 94.43\%$\downarrow$ & 62.36\%$\downarrow$\\

\bottomrule
\end{tabular}
}
    \vspace{-1em}
    \label{tab:motivation_small}
\end{table}

